Time-Sensitive Networking (TSN) for Industrial Automation: Current Advances and Future Directions

With the introduction of Cyber-Physical Systems (CPS) and Internet of Things (IoT) technologies, the automation industry is undergoing significant changes, particularly in improving production efficiency and reducing maintenance costs. Industrial automation applications often need to transmit time- and safety-critical data to closely monitor and control industrial processes. Several Ethernet-based fieldbus solutions, such as PROFINET IRT, EtherNet/IP, and EtherCAT, are widely used to ensure real-time communications in industrial automation systems. These solutions, however, commonly incorporate additional mechanisms to provide latency guarantees, making their interoperability a grand challenge. The IEEE 802.1 Time Sensitive Networking (TSN) task group was formed to enhance and optimize IEEE 802.1 network standards, particularly for Ethernet-based networks. These solutions can be evolved and adapted for cross-industry scenarios, such as large-scale distributed industrial plants requiring multiple industrial entities to work collaboratively. This paper provides a comprehensive review of current advances in TSN standards for industrial automation. It presents the state-of-the-art IEEE TSN standards and discusses the opportunities and challenges of integrating TSN into the automation industry. Some promising research directions are also highlighted for applying TSN technologies to industrial automation applications.

==> sec/TSNOV.tex <==
\section{TSN Overview}
\label{Sec:TSNOV}
% {\color{red} This section aims to provide a TSN overview... to provide a big picture...}
% (From reviewer 3) It fails to describe how to apply the concepts, how they can be used together, and misses many important differences. 

An improved overview including connections between different mechanisms would be a useful contribution, but this paper does not provide that, nor the details necessary to conclude them on your own. There are no lessons learned here. 

(From reviewer 2). Add (i) how exactly the industrial automation is performed with the closed propitiatory technologies. Little more details on this would be useful though you have touched on this. (ii) some detailed example of industrial automation or factory automation to show how various machines sensors, acutators and tools need to work together in a timely manner and how TSN technologies can help.

Why not include the work in AVNU, 3GPP URLLC, and some considerations for IEEE 802.11be?

The introduction/background can be expanded little more as pointed out eariler. It may be also good to show some high-level summary of performance results that are/can be achieved with TSN technologies. 

(From reviewer 1) (i) Focus only on standardization efforts and specifications, and not on first real system solutions implementing part of the emerging standards. (ii) lack of a specific sub-section about ETSI MEC and its role for TSN in future wireless industrial automation solutions; (iii) lack of lessons learned, only standard specification descriptions. 

The technical value and contribution of the manuscript would increase if: (i) including a new sub-section about edge computing (possibly also Multi-access edge computing in 5G) and TSN, which is very relevant topic in the perspectives of the next few years. (ii) including a new section that describes the first implemented solutions that are compliant with some related standard specifications. 

==> sec/abstract.tex <==
With the introduction of Cyber-Physical Systems (CPS) and Internet of Things (IoT) into industrial applications, industrial automation is undergoing tremendous change, especially with regard to improving efficiency and reducing the cost of product. Industrial automation applications are often required to transmit \textit{time-} and \textit{safety-}critical data to monitor and control the industrial processes, especially for critical control systems. There are a number of solutions to meet these requirements (e.g., priority-based real-time schedules and closed-loop feedback control systems). However, due to their different processing capabilities (e.g., in the end devices and network switches), different vendors may come out with distinct solutions, and this makes the large-scale integration of devices from different vendors difficult or impossible. IEEE 802.1 Time-Sensitive Networking (TSN) is a standardization group formed to enhance and optimize the IEEE 802.1 network standards, especially for Ethernet-based networks. These solutions can be evolved and adapted into a cross-industry scenario, such as a large-scale distributed industrial plant, which requires multiple industrial entities working collaboratively. This paper provides a comprehensive review on the current advances in TSN standards for industrial automation. We present the state-of-the-art IEEE TSN standards and discuss the opportunities and challenges when integrating each protocol into the industry domains. Finally, we discuss some promising research about applying the TSN technology to industrial automation applications. 

==> sec/notes.tex <==
{\color{red} Revision Notes (The following two need to be addressed! All others already addressed.)

1. This paper does not include any lessons learned from practical and usage in real/realistic scenarios. ({\color{blue} Explain/planed actions: It seems the journal of IEEE COMST often requires the papers provide a description of lessons learned (I did not find other journals have this requirement). One possible solution to address this is to add one or two paragraphs in each subcategory of four categories at the end of that section, and then marked clearly with ``Lessons Learned on ..."}.)

2. The survey fails to answer important questions: It describes the mechanisms, but it does not describe how to apply them, and what their trade offs in practice actually are. If I have a network with TAS (Qbv) support and a central control unit, how exactly is the GCL of each device configured? What would an appropriate algorithm be for this? If my network only supports CBS (Qav), what are the latency bounds that can actually be given? What is the computation complexity? It is often stated that TAS can provide extremely low latency guarantees together with frame preemption. How low exactly? What does it depend on?

The authors want to list opportunities to apply TSN mechanisms in industrial use cases. Without detailed information on how to use the mechanisms, this can quickly be summarized: "industrial applications need deterministic networking, and TSN can provide deterministic networking". It does currently not provide more information, except for another general introduction into TSN components. In its current state, the paper was surely a lot of work, but it does not present significant new contributions to existing literature. 

A concrete suggestion for improvement: re-organize your presentation. The paper re-visits the same concepts over and over again (e.g., Section II B vs Section IV), without providing in-depth insights. Aggregate your description of the different mechanisms into a single, well-organized description. Think of additional key indicators that describe them beyond their buzzwords that are commonly associated with them. For example, both CBS and ATS enable bounded latency by re-shaping incoming traffic asynchronously. When should CBS be picked, and when ATS? What makes them different? Describe possible usage scenarios. TAS can lead to ultra low latencies - great - how? How does the bridge know what the GCL looks like? What are example centralized or distributed algorithms that configure each of these components? This would actually show opportunities on how to apply each mechanism in a concrete scenario. And this would also reveal a lot more challenges and future research directions.

}
